Unified Out-Of-Distribution Detection: A Model-Specific Perspective

Out-of-distribution (OOD) detection aims to identify test examples that do not belong to the training distribution and are thus unlikely to be predicted reliably. Despite a plethora of existing works, most of them focused only on the scenario where OOD examples come from semantic shift (e.g., unseen categories), ignoring other possible causes (e.g., covariate shift). In this paper, we present a novel, unifying framework to study OOD detection in a broader scope. Instead of detecting OOD examples from a particular cause, we propose to detect examples that a deployed machine learning model (e.g., an image classifier) is unable to predict correctly. That is, whether a test example should be detected and rejected or not is ``model-specific''. We show that this framework unifies the detection of OOD examples caused by semantic shift and covariate shift, and closely addresses the concern of applying a machine learning model to uncontrolled environments. We provide an extensive analysis that involves a variety of models (e.g., different architectures and training strategies), sources of OOD examples, and OOD detection approaches, and reveal several insights into improving and understanding OOD detection in uncontrolled environments.

==> table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{\textbf{C-OOD Detection under MS-OOD Framework} across datasets models}
\centering
\small
\resizebox{14.5cm}{!}{
\begin{tabular}{|ccccccccccccc|}
\hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                          & \multicolumn{2}{c|}{MS-OOD@ID}                                                                            & \multicolumn{9}{c|}{MS-OOD@C-OOD}                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \cline{3-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{}                          & \multicolumn{2}{c|}{IN}                                                                                   & \multicolumn{2}{c|}{IN-V2}                                                                                & \multicolumn{2}{c|}{IN-Sketch}                                                                            & \multicolumn{2}{c|}{IN-R}                                                                                 & \multicolumn{2}{c|}{IN-A}                                                                                 &                                       \\ \cline{3-12}
\multicolumn{1}{|c|}{\multirow{-3}{*}{MODEL}}             & \multicolumn{1}{c|}{\multirow{-3}{*}{METHODS}} & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{FPR95@ID+↓}                            & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{F95↑}                                  & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{F95↑}                                  & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{F95↑}                                  & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{F95↑}                                  & \multirow{-2}{*}{AVG}                 \\ \hline
\multicolumn{13}{|c|}{DEPTH}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{63.38}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.835}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.515}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.623}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.017}                                 & 0.497                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{71.39}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.817}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.525}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.646}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.017}                                 & {\color[HTML]{FF0000} \textbf{0.502}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{75.07}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.811}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.506}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.606}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.014}                                 & 0.484                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{75.07}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.811}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.508}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.606}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.014}                                 & 0.485                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet18}}          & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{69.76}} & \multicolumn{1}{c|}{87.48}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{66.52}} & \multicolumn{1}{c|}{0.790}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{20.23}} & \multicolumn{1}{c|}{0.429}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{33.06}} & \multicolumn{1}{c|}{0.540}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{1.15}}  & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.024}}} & 0.446                                 \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{61.66}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.866}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.557}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.698}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & {\color[HTML]{FF0000} \textbf{0.707}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{70.67}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.853}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.584}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.638}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.692                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{74.86}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.849}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.570}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.604}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.674                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.72}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.838}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.578}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.614}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.677                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}          & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}} & \multicolumn{1}{c|}{89.60}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{0.825}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{0.485}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{0.575}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                   & 0.628                                 \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{60.92}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.879}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.601}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.737}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.129}                                 & {\color[HTML]{FF0000} \textbf{0.587}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{70.56}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.864}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.617}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.652}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.130}}} & 0.566                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{73.45}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.859}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.609}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.626}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.130}                                 & 0.556                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{77.78}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.859}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.615}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.653}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.098}                                 & 0.556                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet152}}         & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{78.31}} & \multicolumn{1}{c|}{91.67}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{75.10}} & \multicolumn{1}{c|}{0.840}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{28.53}} & \multicolumn{1}{c|}{0.512}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{41.34}} & \multicolumn{1}{c|}{0.608}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{6.03}}  & \multicolumn{1}{c|}{0.122}                                 & 0.520                                 \\ \hline
\multicolumn{13}{|c|}{TRAINING}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{61.66}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.866}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.557}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.698}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & {\color[HTML]{FF0000} \textbf{0.707}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{70.67}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.853}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.584}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.638}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.692                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{74.86}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.849}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.570}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.604}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.674                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.72}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.838}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.578}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.614}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.677                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}          & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}} & \multicolumn{1}{c|}{89.60}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{0.825}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{0.485}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{0.575}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                   & 0.628                                 \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{66.52}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.884}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.594}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.754}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.282}}} & {\color[HTML]{FF0000} \textbf{0.628}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.24}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.878}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.562}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.686}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.235}                                 & 0.590                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{94.41}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.856}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.452}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.207}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.072}                                 & 0.397                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{85.10}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.865}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.593}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.633}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.206}                                 & 0.574                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{Robust   ResNet50}} & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{80.86}} & \multicolumn{1}{c|}{99.15}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{77.71}} & \multicolumn{1}{c|}{0.850}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{29.86}} & \multicolumn{1}{c|}{0.458}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{42.82}} & \multicolumn{1}{c|}{0.598}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{14.55}} & \multicolumn{1}{c|}{0.254}                                 & 0.540                                 \\ \hline
\multicolumn{13}{|c|}{PRETRAINING}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{61.66}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.866}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.557}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.698}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & {\color[HTML]{FF0000} \textbf{0.707}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{70.67}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.853}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.584}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.638}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.692                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{74.86}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.849}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.570}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.604}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.674                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.72}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.838}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.578}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.614}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.677                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}          & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}} & \multicolumn{1}{c|}{89.60}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{0.825}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{0.485}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{0.575}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                   & 0.628                                 \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{72.11}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.775}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.631}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.803}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.413}}} & {\color[HTML]{FF0000} \textbf{0.656}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{86.62}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.745}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.531}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.760}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.364}                                 & 0.600                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{90.67}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.739}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.523}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.736}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.349}                                 & 0.587                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{90.74}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.738}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.523}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.733}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.348}                                 & 0.586                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{CLIP-ResNet50}}     & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{59.82}} & \multicolumn{1}{c|}{93.94}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{59.53}} & \multicolumn{1}{c|}{0.734}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{35.50}} & \multicolumn{1}{c|}{0.515}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{60.60}} & \multicolumn{1}{c|}{0.749}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{22.76}} & \multicolumn{1}{c|}{0.375}                                 & 0.593                                 \\ \hline
\multicolumn{13}{|c|}{ARCHITECTURE}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{61.66}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.866}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.557}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.698}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & {\color[HTML]{FF0000} \textbf{0.707}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{70.67}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.853}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.584}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.638}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.692                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{74.86}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.849}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.570}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.604}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.674                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.72}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.838}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.578}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.614}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                      & 0.677                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{13-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}          & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}} & \multicolumn{1}{c|}{89.60}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{0.825}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{0.485}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{0.575}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                   & 0.628                                 \\ \hline
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{59.43}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.889}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.637}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.789}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.388}}} & {\color[HTML]{FF0000} \textbf{0.676}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.89}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.883}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.640}}} & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.698}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.298}                                 & 0.630                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{75.81}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.870}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.623}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.611}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.255}                                 & 0.590                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.26}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.870}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.601}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.596}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.143}                                 & 0.553                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} \cline{12-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ViT-B-16}}          & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{81.07}} & \multicolumn{1}{c|}{98.08}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{77.38}} & \multicolumn{1}{c|}{0.846}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{29.40}} & \multicolumn{1}{c|}{0.469}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{44.00}} & \multicolumn{1}{c|}{0.613}                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{20.84}} & \multicolumn{1}{c|}{0.347}                                 & 0.569                                 \\ \hline
\end{tabular}}
\label{table2}
\end{table*}

==> table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{Difference between the previous and our MS-OOD framework. Please see a full version in~\autoref{table5} with additional datasets.}
\resizebox{14cm}{!}{
\begin{tabular}{|ccccccccccccc|}
\hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{ID}                       & \multicolumn{10}{c|}{S-OOD}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{3-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{IN}                       & \multicolumn{2}{c|}{SVHN}                                                                                                                   & \multicolumn{2}{c|}{DTD}                                                                                                                     & \multicolumn{2}{c|}{SUN}                                                                                                                     & \multicolumn{2}{c|}{SSB-IN-Easy}                                                                                                             & \multicolumn{2}{c|}{AVG}                                                                                                \\ \cline{3-13} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{MODEL}}           & \multicolumn{1}{c|}{\multirow{-3}{*}{METHODS}} & \multicolumn{1}{c|}{ACC↑}                     & \multicolumn{1}{c|}{FPR95↓}                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}} & \multicolumn{1}{c|}{FPR95↓}                                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}} & \multicolumn{1}{c|}{FPR95↓}                                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}} & \multicolumn{1}{c|}{FPR95↓}                                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}} & \multicolumn{1}{c|}{FPR95↓}                                & \begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular} \\ \hline
\multicolumn{13}{|c|}{\textbf{DEPTH}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{10.67}                                & \multicolumn{1}{c|}{2.52}                                                       & \multicolumn{1}{c|}{70.16}                                 & \multicolumn{1}{c|}{46.33}                                                      & \multicolumn{1}{c|}{73.45}                                 & \multicolumn{1}{c|}{47.99}                                                      & \multicolumn{1}{c|}{79.00}                                 & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{54.52}}}                      & \multicolumn{1}{c|}{58.32}                                 & 37.84                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{5.80}                                 & \multicolumn{1}{c|}{1.10}                                                       & \multicolumn{1}{c|}{57.18}                                 & \multicolumn{1}{c|}{36.12}                                                      & \multicolumn{1}{c|}{62.92}                                 & \multicolumn{1}{c|}{39.54}                                                      & \multicolumn{1}{c|}{75.36}                                 & \multicolumn{1}{c|}{54.98}                                                      & \multicolumn{1}{c|}{50.31}                                 & 32.93                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{6.53}                                 & \multicolumn{1}{c|}{1.53}                                                       & \multicolumn{1}{c|}{52.82}                                 & \multicolumn{1}{c|}{36.06}                                                      & \multicolumn{1}{c|}{59.75}                                 & \multicolumn{1}{c|}{39.83}                                                      & \multicolumn{1}{c|}{74.97}                                 & \multicolumn{1}{c|}{57.87}                                                      & \multicolumn{1}{c|}{48.52}                                 & 33.82                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{1.61}                                 & \multicolumn{1}{c|}{0.59}                                                       & \multicolumn{1}{c|}{38.83}                                 & \multicolumn{1}{c|}{26.97}                                                      & \multicolumn{1}{c|}{93.08}                                 & \multicolumn{1}{c|}{87.19}                                                      & \multicolumn{1}{c|}{80.09}                                 & \multicolumn{1}{c|}{68.88}                                                      & \multicolumn{1}{c|}{53.40}                                 & 45.91                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet18}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{69.758}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.29}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.12}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{29.31}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{23.35}}}                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{34.66}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{28.56}}}                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{71.69}}} & \multicolumn{1}{c|}{65.14}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{33.99}}} & {\color[HTML]{FF0000} \textbf{29.29}}                      \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{12.89}                                & \multicolumn{1}{c|}{4.21}                                                       & \multicolumn{1}{c|}{66.01}                                 & \multicolumn{1}{c|}{45.11}                                                      & \multicolumn{1}{c|}{68.58}                                 & \multicolumn{1}{c|}{45.41}                                                      & \multicolumn{1}{c|}{72.57}                                 & \multicolumn{1}{c|}{50.81}                                                      & \multicolumn{1}{c|}{55.01}                                 & 36.39                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{7.46}                                 & \multicolumn{1}{c|}{2.33}                                                       & \multicolumn{1}{c|}{54.36}                                 & \multicolumn{1}{c|}{36.28}                                                      & \multicolumn{1}{c|}{59.90}                                 & \multicolumn{1}{c|}{38.76}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.02}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{50.00}}}                      & \multicolumn{1}{c|}{47.68}                                 & {\color[HTML]{FF0000} \textbf{31.84}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{8.18}                                 & \multicolumn{1}{c|}{2.94}                                                       & \multicolumn{1}{c|}{52.13}                                 & \multicolumn{1}{c|}{37.77}                                                      & \multicolumn{1}{c|}{58.28}                                 & \multicolumn{1}{c|}{41.19}                                                      & \multicolumn{1}{c|}{69.19}                                 & \multicolumn{1}{c|}{53.38}                                                      & \multicolumn{1}{c|}{46.94}                                 & 33.82                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.79}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.16}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{15.74}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{9.10}}}                       & \multicolumn{1}{c|}{82.06}                                 & \multicolumn{1}{c|}{69.65}                                                      & \multicolumn{1}{c|}{76.16}                                 & \multicolumn{1}{c|}{63.29}                                                      & \multicolumn{1}{c|}{43.69}                                 & 35.55                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}}  & \multicolumn{1}{c|}{1.14}                                 & \multicolumn{1}{c|}{0.86}                                                       & \multicolumn{1}{c|}{32.39}                                 & \multicolumn{1}{c|}{29.31}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{37.25}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{33.78}}}                      & \multicolumn{1}{c|}{69.82}                                 & \multicolumn{1}{c|}{66.34}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{35.15}}} & 32.57                                                      \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{25.55}                                & \multicolumn{1}{c|}{10.45}                                                      & \multicolumn{1}{c|}{59.84}                                 & \multicolumn{1}{c|}{42.13}                                                      & \multicolumn{1}{c|}{66.01}                                 & \multicolumn{1}{c|}{45.89}                                                      & \multicolumn{1}{c|}{71.31}                                 & \multicolumn{1}{c|}{51.74}                                                      & \multicolumn{1}{c|}{55.68}                                 & 37.55                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{18.00}                                & \multicolumn{1}{c|}{5.44}                                                       & \multicolumn{1}{c|}{45.59}                                 & \multicolumn{1}{c|}{29.63}                                                      & \multicolumn{1}{c|}{51.87}                                 & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{34.06}}}                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{66.05}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{48.39}}}                      & \multicolumn{1}{c|}{45.38}                                 & {\color[HTML]{FF0000} \textbf{29.38}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{21.51}                                & \multicolumn{1}{c|}{7.24}                                                       & \multicolumn{1}{c|}{43.83}                                 & \multicolumn{1}{c|}{29.52}                                                      & \multicolumn{1}{c|}{50.25}                                 & \multicolumn{1}{c|}{34.73}                                                      & \multicolumn{1}{c|}{66.37}                                 & \multicolumn{1}{c|}{50.58}                                                      & \multicolumn{1}{c|}{45.49}                                 & 30.52                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.27}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.08}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{12.98}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{7.71}}}                       & \multicolumn{1}{c|}{77.76}                                 & \multicolumn{1}{c|}{63.40}                                                      & \multicolumn{1}{c|}{73.54}                                 & \multicolumn{1}{c|}{60.18}                                                      & \multicolumn{1}{c|}{41.14}                                 & 32.84                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet152}}       & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{78.312}} & \multicolumn{1}{c|}{3.49}                                 & \multicolumn{1}{c|}{2.94}                                                       & \multicolumn{1}{c|}{31.91}                                 & \multicolumn{1}{c|}{30.32}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{43.46}}} & \multicolumn{1}{c|}{41.73}                                                      & \multicolumn{1}{c|}{73.99}                                 & \multicolumn{1}{c|}{72.26}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{38.21}}} & 36.81                                                      \\ \hline
\multicolumn{13}{|c|}{\textbf{TRAINING}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{12.89}                                & \multicolumn{1}{c|}{4.21}                                                       & \multicolumn{1}{c|}{66.01}                                 & \multicolumn{1}{c|}{45.11}                                                      & \multicolumn{1}{c|}{68.58}                                 & \multicolumn{1}{c|}{45.41}                                                      & \multicolumn{1}{c|}{72.57}                                 & \multicolumn{1}{c|}{50.81}                                                      & \multicolumn{1}{c|}{55.01}                                 & 36.39                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{7.46}                                 & \multicolumn{1}{c|}{2.33}                                                       & \multicolumn{1}{c|}{54.36}                                 & \multicolumn{1}{c|}{36.28}                                                      & \multicolumn{1}{c|}{59.90}                                 & \multicolumn{1}{c|}{38.76}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.02}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{50.00}}}                      & \multicolumn{1}{c|}{47.68}                                 & {\color[HTML]{FF0000} \textbf{31.84}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{8.18}                                 & \multicolumn{1}{c|}{2.94}                                                       & \multicolumn{1}{c|}{52.13}                                 & \multicolumn{1}{c|}{37.77}                                                      & \multicolumn{1}{c|}{58.28}                                 & \multicolumn{1}{c|}{41.19}                                                      & \multicolumn{1}{c|}{69.19}                                 & \multicolumn{1}{c|}{53.38}                                                      & \multicolumn{1}{c|}{46.94}                                 & 33.82                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.79}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.16}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{15.74}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{9.10}}}                       & \multicolumn{1}{c|}{82.06}                                 & \multicolumn{1}{c|}{69.65}                                                      & \multicolumn{1}{c|}{76.16}                                 & \multicolumn{1}{c|}{63.29}                                                      & \multicolumn{1}{c|}{43.69}                                 & 35.55                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}}  & \multicolumn{1}{c|}{1.14}                                 & \multicolumn{1}{c|}{0.86}                                                       & \multicolumn{1}{c|}{32.39}                                 & \multicolumn{1}{c|}{29.31}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{37.25}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{33.78}}}                      & \multicolumn{1}{c|}{69.82}                                 & \multicolumn{1}{c|}{66.34}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{35.15}}} & 32.57                                                      \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{38.41}                                & \multicolumn{1}{c|}{20.77}                                                      & \multicolumn{1}{c|}{71.91}                                 & \multicolumn{1}{c|}{56.22}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{70.86}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{53.12}}}                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{72.80}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{56.58}}}                      & \multicolumn{1}{c|}{63.50}                                 & 46.68                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{54.31}                                & \multicolumn{1}{c|}{37.01}                                                      & \multicolumn{1}{c|}{75.43}                                 & \multicolumn{1}{c|}{64.26}                                                      & \multicolumn{1}{c|}{75.04}                                 & \multicolumn{1}{c|}{62.21}                                                      & \multicolumn{1}{c|}{75.75}                                 & \multicolumn{1}{c|}{63.82}                                                      & \multicolumn{1}{c|}{70.13}                                 & 56.82                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{99.98}                                & \multicolumn{1}{c|}{99.97}                                                      & \multicolumn{1}{c|}{95.74}                                 & \multicolumn{1}{c|}{95.64}                                                      & \multicolumn{1}{c|}{97.72}                                 & \multicolumn{1}{c|}{97.62}                                                      & \multicolumn{1}{c|}{95.59}                                 & \multicolumn{1}{c|}{95.46}                                                      & \multicolumn{1}{c|}{97.26}                                 & 97.17                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.07}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.03}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{21.91}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{18.72}}}                      & \multicolumn{1}{c|}{73.30}                                 & \multicolumn{1}{c|}{67.25}                                                      & \multicolumn{1}{c|}{73.87}                                 & \multicolumn{1}{c|}{67.45}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{42.29}}} & {\color[HTML]{FF0000} \textbf{38.36}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{Robust ResNet50}} & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{80.856}} & \multicolumn{1}{c|}{100.00}                               & \multicolumn{1}{c|}{100.00}                                                     & \multicolumn{1}{c|}{97.45}                                 & \multicolumn{1}{c|}{97.77}                                                      & \multicolumn{1}{c|}{99.76}                                 & \multicolumn{1}{c|}{99.81}                                                      & \multicolumn{1}{c|}{99.49}                                 & \multicolumn{1}{c|}{99.58}                                                      & \multicolumn{1}{c|}{99.17}                                 & 99.29                                                      \\ \hline
\multicolumn{13}{|c|}{\textbf{CLIP}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{12.89}                                & \multicolumn{1}{c|}{4.21}                                                       & \multicolumn{1}{c|}{66.01}                                 & \multicolumn{1}{c|}{45.11}                                                      & \multicolumn{1}{c|}{68.58}                                 & \multicolumn{1}{c|}{45.41}                                                      & \multicolumn{1}{c|}{72.57}                                 & \multicolumn{1}{c|}{50.81}                                                      & \multicolumn{1}{c|}{55.01}                                 & 36.39                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{7.46}                                 & \multicolumn{1}{c|}{2.33}                                                       & \multicolumn{1}{c|}{54.36}                                 & \multicolumn{1}{c|}{36.28}                                                      & \multicolumn{1}{c|}{59.90}                                 & \multicolumn{1}{c|}{38.76}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.02}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{50.00}}}                      & \multicolumn{1}{c|}{47.68}                                 & {\color[HTML]{FF0000} \textbf{31.84}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{8.18}                                 & \multicolumn{1}{c|}{2.94}                                                       & \multicolumn{1}{c|}{52.13}                                 & \multicolumn{1}{c|}{37.77}                                                      & \multicolumn{1}{c|}{58.28}                                 & \multicolumn{1}{c|}{41.19}                                                      & \multicolumn{1}{c|}{69.19}                                 & \multicolumn{1}{c|}{53.38}                                                      & \multicolumn{1}{c|}{46.94}                                 & 33.82                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.79}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.16}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{15.74}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{9.10}}}                       & \multicolumn{1}{c|}{82.06}                                 & \multicolumn{1}{c|}{69.65}                                                      & \multicolumn{1}{c|}{76.16}                                 & \multicolumn{1}{c|}{63.29}                                                      & \multicolumn{1}{c|}{43.69}                                 & 35.55                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}}  & \multicolumn{1}{c|}{1.14}                                 & \multicolumn{1}{c|}{0.86}                                                       & \multicolumn{1}{c|}{32.39}                                 & \multicolumn{1}{c|}{29.31}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{37.25}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{33.78}}}                      & \multicolumn{1}{c|}{69.82}                                 & \multicolumn{1}{c|}{66.34}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{35.15}}} & 32.57                                                      \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{10.29}                                & \multicolumn{1}{c|}{4.24}                                                       & \multicolumn{1}{c|}{66.76}                                 & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{46.65}}}                      & \multicolumn{1}{c|}{70.83}                                 & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{48.72}}}                      & \multicolumn{1}{c|}{80.08}                                 & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{60.29}}}                      & \multicolumn{1}{c|}{56.99}                                 & {\color[HTML]{FF0000} \textbf{39.98}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{61.22}                                & \multicolumn{1}{c|}{29.34}                                                      & \multicolumn{1}{c|}{89.52}                                 & \multicolumn{1}{c|}{82.55}                                                      & \multicolumn{1}{c|}{69.12}                                 & \multicolumn{1}{c|}{53.47}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{77.91}}} & \multicolumn{1}{c|}{68.30}                                                      & \multicolumn{1}{c|}{74.44}                                 & 58.42                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{97.11}                                & \multicolumn{1}{c|}{94.22}                                                      & \multicolumn{1}{c|}{94.36}                                 & \multicolumn{1}{c|}{92.34}                                                      & \multicolumn{1}{c|}{79.59}                                 & \multicolumn{1}{c|}{72.20}                                                      & \multicolumn{1}{c|}{81.20}                                 & \multicolumn{1}{c|}{76.74}                                                      & \multicolumn{1}{c|}{88.07}                                 & 83.87                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{96.72}                                & \multicolumn{1}{c|}{93.43}                                                      & \multicolumn{1}{c|}{94.68}                                 & \multicolumn{1}{c|}{92.71}                                                      & \multicolumn{1}{c|}{81.75}                                 & \multicolumn{1}{c|}{74.12}                                                      & \multicolumn{1}{c|}{81.70}                                 & \multicolumn{1}{c|}{77.03}                                                      & \multicolumn{1}{c|}{88.71}                                 & 84.32                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{CLIP-ResNet50}}   & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{59.818}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.01}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.01}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{48.30}}} & \multicolumn{1}{c|}{46.70}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{60.59}}} & \multicolumn{1}{c|}{58.38}                                                      & \multicolumn{1}{c|}{84.04}                                 & \multicolumn{1}{c|}{83.02}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{48.23}}} & 47.03                                                      \\ \hline
\multicolumn{13}{|c|}{ARCHITECTURE}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{12.89}                                & \multicolumn{1}{c|}{4.21}                                                       & \multicolumn{1}{c|}{66.01}                                 & \multicolumn{1}{c|}{45.11}                                                      & \multicolumn{1}{c|}{68.58}                                 & \multicolumn{1}{c|}{45.41}                                                      & \multicolumn{1}{c|}{72.57}                                 & \multicolumn{1}{c|}{50.81}                                                      & \multicolumn{1}{c|}{55.01}                                 & 36.39                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{7.46}                                 & \multicolumn{1}{c|}{2.33}                                                       & \multicolumn{1}{c|}{54.36}                                 & \multicolumn{1}{c|}{36.28}                                                      & \multicolumn{1}{c|}{59.90}                                 & \multicolumn{1}{c|}{38.76}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.02}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{50.00}}}                      & \multicolumn{1}{c|}{47.68}                                 & {\color[HTML]{FF0000} \textbf{31.84}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{8.18}                                 & \multicolumn{1}{c|}{2.94}                                                       & \multicolumn{1}{c|}{52.13}                                 & \multicolumn{1}{c|}{37.77}                                                      & \multicolumn{1}{c|}{58.28}                                 & \multicolumn{1}{c|}{41.19}                                                      & \multicolumn{1}{c|}{69.19}                                 & \multicolumn{1}{c|}{53.38}                                                      & \multicolumn{1}{c|}{46.94}                                 & 33.82                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.79}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.16}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{15.74}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{9.10}}}                       & \multicolumn{1}{c|}{82.06}                                 & \multicolumn{1}{c|}{69.65}                                                      & \multicolumn{1}{c|}{76.16}                                 & \multicolumn{1}{c|}{63.29}                                                      & \multicolumn{1}{c|}{43.69}                                 & 35.55                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{76.13}}  & \multicolumn{1}{c|}{1.14}                                 & \multicolumn{1}{c|}{0.86}                                                       & \multicolumn{1}{c|}{32.39}                                 & \multicolumn{1}{c|}{29.31}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{37.25}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{33.78}}}                      & \multicolumn{1}{c|}{69.82}                                 & \multicolumn{1}{c|}{66.34}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{35.15}}} & 32.57                                                      \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{21.54}                                & \multicolumn{1}{c|}{10.09}                                                      & \multicolumn{1}{c|}{58.30}                                 & \multicolumn{1}{c|}{41.28}                                                      & \multicolumn{1}{c|}{66.56}                                 & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{48.08}}}                      & \multicolumn{1}{c|}{71.31}                                 & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{53.54}}}                      & \multicolumn{1}{c|}{54.43}                                 & 38.25                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{18.52}                                & \multicolumn{1}{c|}{8.23}                                                       & \multicolumn{1}{c|}{54.84}                                 & \multicolumn{1}{c|}{38.09}                                                      & \multicolumn{1}{c|}{66.89}                                 & \multicolumn{1}{c|}{49.91}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{70.17}}} & \multicolumn{1}{c|}{54.13}                                                      & \multicolumn{1}{c|}{52.60}                                 & 37.59                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{24.15}                                & \multicolumn{1}{c|}{13.50}                                                      & \multicolumn{1}{c|}{57.39}                                 & \multicolumn{1}{c|}{46.01}                                                      & \multicolumn{1}{c|}{72.77}                                 & \multicolumn{1}{c|}{62.80}                                                      & \multicolumn{1}{c|}{73.77}                                 & \multicolumn{1}{c|}{63.99}                                                      & \multicolumn{1}{c|}{57.02}                                 & 46.58                                                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{2.34}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{0.85}}}                       & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{43.94}}} & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{31.49}}}                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{59.46}}} & \multicolumn{1}{c|}{49.05}                                                      & \multicolumn{1}{c|}{71.58}                                 & \multicolumn{1}{c|}{58.70}                                                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{44.33}}} & {\color[HTML]{FF0000} \textbf{35.02}}                      \\ \cline{2-2} \cline{4-13} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ViT-B-16}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{81.068}} & \multicolumn{1}{c|}{96.13}                                & \multicolumn{1}{c|}{96.43}                                                      & \multicolumn{1}{c|}{92.87}                                 & \multicolumn{1}{c|}{93.14}                                                      & \multicolumn{1}{c|}{96.85}                                 & \multicolumn{1}{c|}{97.05}                                                      & \multicolumn{1}{c|}{97.86}                                 & \multicolumn{1}{c|}{98.04}                                                      & \multicolumn{1}{c|}{95.93}                                 & 96.16                                                      \\ \hline
\end{tabular}}
\label{table3}
\end{table*}

==> table4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\small
\centering
\caption{C-OOD detection under MS-OOD Framework only on C-OOD dataset}
\resizebox{15cm}{!}{
\begin{tabular}{|ccccccccccc|}
\hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{}                          & \multicolumn{9}{c|}{MS-ID@COOD vs   MS-OOD@COOD}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \cline{3-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{}                          & \multicolumn{2}{c|}{IN-V2}                                                                                                       & \multicolumn{2}{c|}{IN-Sketch}                                                                                                   & \multicolumn{2}{c|}{IN-R}                                                                                                        & \multicolumn{2}{c|}{IN-A}                                                                                                        &                                       \\ \cline{3-10}
\multicolumn{1}{|c|}{\multirow{-3}{*}{MODEL}}           & \multicolumn{1}{c|}{\multirow{-3}{*}{METHODS}} & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @COOD+↓\end{tabular}} & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @COOD+↓\end{tabular}} & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @COOD+↓\end{tabular}} & \multicolumn{1}{c|}{ACC↑}                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FPR95\\      @COOD+↓\end{tabular}} & \multirow{-2}{*}{AVG}                 \\ \hline
\multicolumn{11}{|c|}{\textbf{DEPTH}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{64.85}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{66.86}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{69.20}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{95.04}                                                        & {\color[HTML]{FF0000} \textbf{73.99}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{74.61}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{68.59}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{68.97}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{95.44}                                                        & 76.90                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.32}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.78}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{71.65}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{96.98}                                                        & 79.93                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{83.75}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{87.15}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{81.97}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{93.35}                                                        & 86.56                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet18}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{66.52}} & \multicolumn{1}{c|}{88.17}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{20.23}} & \multicolumn{1}{c|}{76.41}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{33.06}} & \multicolumn{1}{c|}{83.62}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{1.15}}  & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{92.03}}}                        & 85.06                                 \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{64.42}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{69.66}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.36}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & {\color[HTML]{FF0000} \textbf{65.81}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.47}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{62.85}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 68.35                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.37}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.97}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{65.57}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 71.64                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{81.83}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.94}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 79.17                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{90.30}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{74.10}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{82.56}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                                          & 82.32                                 \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{62.93}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{66.45}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{60.35}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{87.42}}}                        & {\color[HTML]{FF0000} \textbf{69.29}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{73.37}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{67.12}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{60.69}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{88.76}                                                        & 72.49                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{77.27}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{70.71}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.12}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{88.69}                                                        & 74.95                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{79.04}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{75.61}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.11}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{94.65}                                                        & 80.35                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet152}}       & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{75.10}} & \multicolumn{1}{c|}{92.09}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{28.53}} & \multicolumn{1}{c|}{76.05}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{41.34}} & \multicolumn{1}{c|}{84.43}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{6.03}}  & \multicolumn{1}{c|}{90.57}                                                        & 85.79                                 \\ \hline
\multicolumn{11}{|c|}{\textbf{TRAINING}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{64.42}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{69.66}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.36}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & {\color[HTML]{FF0000} \textbf{65.81}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.47}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{62.85}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 68.35                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.37}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.97}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{65.57}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 71.64                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{81.83}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.94}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 79.17                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{90.30}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{74.10}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{82.56}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                                          & 82.32                                 \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.00}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{71.23}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{61.37}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{88.75}}}                        & {\color[HTML]{FF0000} \textbf{72.59}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.77}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{75.30}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{61.42}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{89.89}                                                        & 74.85                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{94.03}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{95.84}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{66.21}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{91.76}                                                        & 86.96                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{85.42}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{75.19}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{74.19}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{91.42}                                                        & 81.56                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{Robust ResNet50}} & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{77.71}} & \multicolumn{1}{c|}{99.19}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{29.86}} & \multicolumn{1}{c|}{98.87}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{42.82}} & \multicolumn{1}{c|}{99.64}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{14.55}} & \multicolumn{1}{c|}{96.52}                                                        & 98.56                                 \\ \hline
\multicolumn{11}{|c|}{\textbf{PRETRAINING}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{64.42}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{69.66}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.36}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & {\color[HTML]{FF0000} \textbf{65.81}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.47}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{62.85}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 68.35                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.37}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.97}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{65.57}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 71.64                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{81.83}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.94}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 79.17                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{90.30}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{74.10}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{82.56}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                                          & 82.32                                 \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{73.61}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{72.81}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{65.92}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{84.64}}}                        & {\color[HTML]{FF0000} \textbf{74.25}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{87.82}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{87.22}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{81.98}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{92.94}                                                        & 87.49                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{91.35}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{93.58}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{88.05}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{94.34}                                                        & 91.83                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{91.52}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{93.67}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{88.29}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{94.67}                                                        & 92.04                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{CLIP-ResNet50}}   & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{59.53}} & \multicolumn{1}{c|}{93.65}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{35.50}} & \multicolumn{1}{c|}{91.77}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{60.60}} & \multicolumn{1}{c|}{88.82}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{22.76}} & \multicolumn{1}{c|}{92.91}                                                        & 91.79                                 \\ \hline
\multicolumn{11}{|c|}{\textbf{ARCHITECTURE}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{64.42}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{69.66}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.36}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & {\color[HTML]{FF0000} \textbf{65.81}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{69.47}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{62.85}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 68.35                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.37}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{72.97}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{65.57}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 71.64                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{81.83}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{78.94}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.74}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                                             & 79.17                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{11-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ResNet50}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{72.37}} & \multicolumn{1}{c|}{90.30}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{24.09}} & \multicolumn{1}{c|}{74.10}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{36.17}} & \multicolumn{1}{c|}{82.56}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{0.00}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{X}}                                          & 82.32                                 \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MSP}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{63.97}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.00}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{57.39}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{87.35}}}                        & {\color[HTML]{FF0000} \textbf{67.93}} \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{MaxLogit}                  & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{67.73}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{{\color[HTML]{FF0000} \textbf{61.90}}}                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{57.81}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{88.46}                                                        & 68.98                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{Energy}                    & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{77.37}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.84}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{59.18}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{90.13}                                                        & 72.63                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{ViM}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{76.88}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{63.73}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{58.80}                                                        & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{90.23}                                                        & 72.41                                 \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-11} 
\multicolumn{1}{|c|}{\multirow{-5}{*}{ViT-B-16}}        & \multicolumn{1}{c|}{GradNorm}                  & \multicolumn{1}{c|}{\multirow{-5}{*}{77.38}} & \multicolumn{1}{c|}{98.59}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{29.40}} & \multicolumn{1}{c|}{83.71}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{44.00}} & \multicolumn{1}{c|}{91.45}                                                        & \multicolumn{1}{c|}{\multirow{-5}{*}{20.84}} & \multicolumn{1}{c|}{92.44}                                                        & 91.55                                 \\ \hline
\end{tabular}}
\label{table4}
\end{table*}

==> table5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{sidewaystable}
\centering
\caption{Appendix: Complete table of \autoref{table3}.}
\resizebox{22cm}{!}{
\begin{tabular}{|ccccccccccccccccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{MODEL}}}           & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{METHODS}}} & \multicolumn{1}{c|}{\textbf{ID}}             & \multicolumn{16}{c|}{\textbf{S-OOD}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\textbf{IN}}             & \multicolumn{2}{c|}{\textbf{SVHN}}                                                                                              & \multicolumn{2}{c|}{\textbf{DTD}}                                                                                               & \multicolumn{2}{c|}{\textbf{Places365}}                                                                                         & \multicolumn{2}{c|}{\textbf{iNaturalist}}                                                                                       & \multicolumn{2}{c|}{\textbf{SUN}}                                                                                               & \multicolumn{2}{c|}{\textbf{IN-O}}                                                                                              & \multicolumn{2}{c|}{\textbf{SSB-IN-Easy}}                                                                                       & \multicolumn{2}{c|}{\textbf{AVG}}                                                                          \\ \cline{3-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\textbf{ACC↑}}           & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}}} & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}}} & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}}} & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}}} & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}}} & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}}} & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}}} & \multicolumn{1}{c|}{\textbf{FPR95↓}} & \textbf{\begin{tabular}[c]{@{}c@{}}FPR95\\      @ID+↓\end{tabular}} \\ \hline
\multicolumn{19}{|c|}{\textbf{DEPTH}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{ResNet18}}}        & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{69.76}} & \multicolumn{1}{c|}{10.67}           & \multicolumn{1}{c|}{2.52}                                                                & \multicolumn{1}{c|}{70.16}           & \multicolumn{1}{c|}{46.33}                                                               & \multicolumn{1}{c|}{75.93}           & \multicolumn{1}{c|}{50.95}                                                               & \multicolumn{1}{c|}{58.22}           & \multicolumn{1}{c|}{30.67}                                                               & \multicolumn{1}{c|}{73.45}           & \multicolumn{1}{c|}{47.99}                                                               & \multicolumn{1}{c|}{99.65}           & \multicolumn{1}{c|}{97.80}                                                               & \multicolumn{1}{c|}{79.00}           & \multicolumn{1}{c|}{\textbf{54.52}}                                                      & \multicolumn{1}{c|}{66.73}           & 47.25                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{5.80}            & \multicolumn{1}{c|}{1.10}                                                                & \multicolumn{1}{c|}{57.18}           & \multicolumn{1}{c|}{36.12}                                                               & \multicolumn{1}{c|}{66.94}           & \multicolumn{1}{c|}{45.25}                                                               & \multicolumn{1}{c|}{54.51}           & \multicolumn{1}{c|}{29.47}                                                               & \multicolumn{1}{c|}{62.92}           & \multicolumn{1}{c|}{39.54}                                                               & \multicolumn{1}{c|}{96.80}           & \multicolumn{1}{c|}{89.90}                                                               & \multicolumn{1}{c|}{75.36}           & \multicolumn{1}{c|}{54.98}                                                               & \multicolumn{1}{c|}{59.93}           & 42.34                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{6.53}            & \multicolumn{1}{c|}{1.53}                                                                & \multicolumn{1}{c|}{52.82}           & \multicolumn{1}{c|}{36.06}                                                               & \multicolumn{1}{c|}{64.97}           & \multicolumn{1}{c|}{46.23}                                                               & \multicolumn{1}{c|}{56.49}           & \multicolumn{1}{c|}{33.70}                                                               & \multicolumn{1}{c|}{59.75}           & \multicolumn{1}{c|}{39.83}                                                               & \multicolumn{1}{c|}{93.15}           & \multicolumn{1}{c|}{85.75}                                                               & \multicolumn{1}{c|}{74.97}           & \multicolumn{1}{c|}{57.87}                                                               & \multicolumn{1}{c|}{58.38}           & 43.00                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{1.61}            & \multicolumn{1}{c|}{0.59}                                                                & \multicolumn{1}{c|}{38.83}           & \multicolumn{1}{c|}{26.97}                                                               & \multicolumn{1}{c|}{92.47}           & \multicolumn{1}{c|}{85.94}                                                               & \multicolumn{1}{c|}{91.15}           & \multicolumn{1}{c|}{83.67}                                                               & \multicolumn{1}{c|}{93.08}           & \multicolumn{1}{c|}{87.19}                                                               & \multicolumn{1}{c|}{\textbf{72.70}}  & \multicolumn{1}{c|}{\textbf{64.00}}                                                      & \multicolumn{1}{c|}{80.09}           & \multicolumn{1}{c|}{68.88}                                                               & \multicolumn{1}{c|}{67.13}           & 59.61                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.29}}   & \multicolumn{1}{c|}{\textbf{0.12}}                                                       & \multicolumn{1}{c|}{\textbf{29.31}}  & \multicolumn{1}{c|}{\textbf{23.35}}                                                      & \multicolumn{1}{c|}{\textbf{45.48}}  & \multicolumn{1}{c|}{\textbf{38.93}}                                                      & \multicolumn{1}{c|}{\textbf{26.76}}  & \multicolumn{1}{c|}{\textbf{21.22}}                                                      & \multicolumn{1}{c|}{\textbf{34.66}}  & \multicolumn{1}{c|}{\textbf{28.56}}                                                      & \multicolumn{1}{c|}{89.25}           & \multicolumn{1}{c|}{85.50}                                                               & \multicolumn{1}{c|}{\textbf{71.69}}  & \multicolumn{1}{c|}{65.14}                                                               & \multicolumn{1}{c|}{\textbf{42.49}}  & \textbf{37.55}                                                      \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{ResNet50}}}        & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{76.13}}  & \multicolumn{1}{c|}{12.89}           & \multicolumn{1}{c|}{4.21}                                                                & \multicolumn{1}{c|}{66.01}           & \multicolumn{1}{c|}{45.11}                                                               & \multicolumn{1}{c|}{71.57}           & \multicolumn{1}{c|}{48.78}                                                               & \multicolumn{1}{c|}{52.77}           & \multicolumn{1}{c|}{29.58}                                                               & \multicolumn{1}{c|}{68.58}           & \multicolumn{1}{c|}{45.41}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{72.57}           & \multicolumn{1}{c|}{50.81}                                                               & \multicolumn{1}{c|}{63.48}           & 46.27                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{7.46}            & \multicolumn{1}{c|}{2.33}                                                                & \multicolumn{1}{c|}{54.36}           & \multicolumn{1}{c|}{36.28}                                                               & \multicolumn{1}{c|}{65.68}           & \multicolumn{1}{c|}{46.18}                                                               & \multicolumn{1}{c|}{50.87}           & \multicolumn{1}{c|}{26.75}                                                               & \multicolumn{1}{c|}{59.90}           & \multicolumn{1}{c|}{38.76}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{\textbf{69.02}}  & \multicolumn{1}{c|}{\textbf{50.00}}                                                      & \multicolumn{1}{c|}{58.18}           & 42.90                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{8.18}            & \multicolumn{1}{c|}{2.94}                                                                & \multicolumn{1}{c|}{52.13}           & \multicolumn{1}{c|}{37.77}                                                               & \multicolumn{1}{c|}{65.40}           & \multicolumn{1}{c|}{48.91}                                                               & \multicolumn{1}{c|}{53.95}           & \multicolumn{1}{c|}{32.48}                                                               & \multicolumn{1}{c|}{58.28}           & \multicolumn{1}{c|}{41.19}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{99.90}                                                               & \multicolumn{1}{c|}{69.19}           & \multicolumn{1}{c|}{53.38}                                                               & \multicolumn{1}{c|}{58.16}           & 45.22                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.79}}   & \multicolumn{1}{c|}{\textbf{0.16}}                                                       & \multicolumn{1}{c|}{\textbf{15.74}}  & \multicolumn{1}{c|}{\textbf{9.10}}                                                       & \multicolumn{1}{c|}{83.52}           & \multicolumn{1}{c|}{72.38}                                                               & \multicolumn{1}{c|}{71.78}           & \multicolumn{1}{c|}{55.45}                                                               & \multicolumn{1}{c|}{82.06}           & \multicolumn{1}{c|}{69.65}                                                               & \multicolumn{1}{c|}{\textbf{84.90}}  & \multicolumn{1}{c|}{\textbf{79.20}}                                                      & \multicolumn{1}{c|}{76.16}           & \multicolumn{1}{c|}{63.29}                                                               & \multicolumn{1}{c|}{59.28}           & 49.89                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{1.14}            & \multicolumn{1}{c|}{0.86}                                                                & \multicolumn{1}{c|}{32.39}           & \multicolumn{1}{c|}{29.31}                                                               & \multicolumn{1}{c|}{\textbf{48.69}}  & \multicolumn{1}{c|}{\textbf{44.80}}                                                      & \multicolumn{1}{c|}{\textbf{26.95}}  & \multicolumn{1}{c|}{\textbf{23.71}}                                                      & \multicolumn{1}{c|}{\textbf{37.25}}  & \multicolumn{1}{c|}{\textbf{33.78}}                                                      & \multicolumn{1}{c|}{95.60}           & \multicolumn{1}{c|}{94.35}                                                               & \multicolumn{1}{c|}{69.82}           & \multicolumn{1}{c|}{66.34}                                                               & \multicolumn{1}{c|}{\textbf{44.55}}  & \textbf{41.88}                                                      \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{ResNet152}}}       & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{78.31}} & \multicolumn{1}{c|}{25.55}           & \multicolumn{1}{c|}{10.45}                                                               & \multicolumn{1}{c|}{59.84}           & \multicolumn{1}{c|}{42.13}                                                               & \multicolumn{1}{c|}{68.93}           & \multicolumn{1}{c|}{48.38}                                                               & \multicolumn{1}{c|}{49.26}           & \multicolumn{1}{c|}{30.33}                                                               & \multicolumn{1}{c|}{66.01}           & \multicolumn{1}{c|}{45.89}                                                               & \multicolumn{1}{c|}{99.30}           & \multicolumn{1}{c|}{96.95}                                                               & \multicolumn{1}{c|}{71.31}           & \multicolumn{1}{c|}{51.74}                                                               & \multicolumn{1}{c|}{62.89}           & 46.55                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{18.00}           & \multicolumn{1}{c|}{5.44}                                                                & \multicolumn{1}{c|}{45.59}           & \multicolumn{1}{c|}{29.63}                                                               & \multicolumn{1}{c|}{58.72}           & \multicolumn{1}{c|}{\textbf{40.23}}                                                      & \multicolumn{1}{c|}{46.31}           & \multicolumn{1}{c|}{\textbf{26.85}}                                                      & \multicolumn{1}{c|}{51.87}           & \multicolumn{1}{c|}{\textbf{34.06}}                                                      & \multicolumn{1}{c|}{96.15}           & \multicolumn{1}{c|}{89.55}                                                               & \multicolumn{1}{c|}{\textbf{66.05}}  & \multicolumn{1}{c|}{\textbf{48.39}}                                                      & \multicolumn{1}{c|}{54.67}           & \textbf{39.16}                                                      \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{21.51}           & \multicolumn{1}{c|}{7.24}                                                                & \multicolumn{1}{c|}{43.83}           & \multicolumn{1}{c|}{29.52}                                                               & \multicolumn{1}{c|}{57.71}           & \multicolumn{1}{c|}{41.65}                                                               & \multicolumn{1}{c|}{49.36}           & \multicolumn{1}{c|}{30.65}                                                               & \multicolumn{1}{c|}{50.25}           & \multicolumn{1}{c|}{34.73}                                                               & \multicolumn{1}{c|}{93.70}           & \multicolumn{1}{c|}{88.05}                                                               & \multicolumn{1}{c|}{66.37}           & \multicolumn{1}{c|}{50.58}                                                               & \multicolumn{1}{c|}{54.68}           & 40.35                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.27}}   & \multicolumn{1}{c|}{\textbf{0.08}}                                                       & \multicolumn{1}{c|}{\textbf{12.98}}  & \multicolumn{1}{c|}{\textbf{7.71}}                                                       & \multicolumn{1}{c|}{78.58}           & \multicolumn{1}{c|}{64.66}                                                               & \multicolumn{1}{c|}{63.14}           & \multicolumn{1}{c|}{43.97}                                                               & \multicolumn{1}{c|}{77.76}           & \multicolumn{1}{c|}{63.40}                                                               & \multicolumn{1}{c|}{\textbf{71.45}}  & \multicolumn{1}{c|}{\textbf{61.20}}                                                      & \multicolumn{1}{c|}{73.54}           & \multicolumn{1}{c|}{60.18}                                                               & \multicolumn{1}{c|}{53.96}           & 43.03                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{3.49}            & \multicolumn{1}{c|}{2.94}                                                                & \multicolumn{1}{c|}{31.91}           & \multicolumn{1}{c|}{30.32}                                                               & \multicolumn{1}{c|}{\textbf{55.87}}  & \multicolumn{1}{c|}{53.69}                                                               & \multicolumn{1}{c|}{\textbf{37.53}}  & \multicolumn{1}{c|}{35.50}                                                               & \multicolumn{1}{c|}{\textbf{43.46}}  & \multicolumn{1}{c|}{41.73}                                                               & \multicolumn{1}{c|}{91.30}           & \multicolumn{1}{c|}{89.90}                                                               & \multicolumn{1}{c|}{73.99}           & \multicolumn{1}{c|}{72.26}                                                               & \multicolumn{1}{c|}{\textbf{48.22}}  & 46.62                                                               \\ \hline
\multicolumn{19}{|c|}{\textbf{TRAINING}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{ResNet50}}}        & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{76.13}}  & \multicolumn{1}{c|}{12.89}           & \multicolumn{1}{c|}{4.21}                                                                & \multicolumn{1}{c|}{66.01}           & \multicolumn{1}{c|}{45.11}                                                               & \multicolumn{1}{c|}{71.57}           & \multicolumn{1}{c|}{48.78}                                                               & \multicolumn{1}{c|}{52.77}           & \multicolumn{1}{c|}{29.58}                                                               & \multicolumn{1}{c|}{68.58}           & \multicolumn{1}{c|}{45.41}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{72.57}           & \multicolumn{1}{c|}{50.81}                                                               & \multicolumn{1}{c|}{63.48}           & 46.27                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{7.46}            & \multicolumn{1}{c|}{2.33}                                                                & \multicolumn{1}{c|}{54.36}           & \multicolumn{1}{c|}{36.28}                                                               & \multicolumn{1}{c|}{65.68}           & \multicolumn{1}{c|}{46.18}                                                               & \multicolumn{1}{c|}{50.87}           & \multicolumn{1}{c|}{26.75}                                                               & \multicolumn{1}{c|}{59.90}           & \multicolumn{1}{c|}{38.76}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{\textbf{69.02}}  & \multicolumn{1}{c|}{\textbf{50.00}}                                                      & \multicolumn{1}{c|}{58.18}           & 42.90                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{8.18}            & \multicolumn{1}{c|}{2.94}                                                                & \multicolumn{1}{c|}{52.13}           & \multicolumn{1}{c|}{37.77}                                                               & \multicolumn{1}{c|}{65.40}           & \multicolumn{1}{c|}{48.91}                                                               & \multicolumn{1}{c|}{53.95}           & \multicolumn{1}{c|}{32.48}                                                               & \multicolumn{1}{c|}{58.28}           & \multicolumn{1}{c|}{41.19}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{99.90}                                                               & \multicolumn{1}{c|}{69.19}           & \multicolumn{1}{c|}{53.38}                                                               & \multicolumn{1}{c|}{58.16}           & 45.22                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.79}}   & \multicolumn{1}{c|}{\textbf{0.16}}                                                       & \multicolumn{1}{c|}{\textbf{15.74}}  & \multicolumn{1}{c|}{\textbf{9.10}}                                                       & \multicolumn{1}{c|}{83.52}           & \multicolumn{1}{c|}{72.38}                                                               & \multicolumn{1}{c|}{71.78}           & \multicolumn{1}{c|}{55.45}                                                               & \multicolumn{1}{c|}{82.06}           & \multicolumn{1}{c|}{69.65}                                                               & \multicolumn{1}{c|}{\textbf{84.90}}  & \multicolumn{1}{c|}{\textbf{79.20}}                                                      & \multicolumn{1}{c|}{76.16}           & \multicolumn{1}{c|}{63.29}                                                               & \multicolumn{1}{c|}{59.28}           & 49.89                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{1.14}            & \multicolumn{1}{c|}{0.86}                                                                & \multicolumn{1}{c|}{32.39}           & \multicolumn{1}{c|}{29.31}                                                               & \multicolumn{1}{c|}{\textbf{48.69}}  & \multicolumn{1}{c|}{\textbf{44.80}}                                                      & \multicolumn{1}{c|}{\textbf{26.95}}  & \multicolumn{1}{c|}{\textbf{23.71}}                                                      & \multicolumn{1}{c|}{\textbf{37.25}}  & \multicolumn{1}{c|}{\textbf{33.78}}                                                      & \multicolumn{1}{c|}{95.60}           & \multicolumn{1}{c|}{94.35}                                                               & \multicolumn{1}{c|}{69.82}           & \multicolumn{1}{c|}{66.34}                                                               & \multicolumn{1}{c|}{\textbf{44.55}}  & \textbf{41.88}                                                      \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{Robust ResNet50}}} & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{80.86}} & \multicolumn{1}{c|}{38.41}           & \multicolumn{1}{c|}{20.77}                                                               & \multicolumn{1}{c|}{71.91}           & \multicolumn{1}{c|}{56.22}                                                               & \multicolumn{1}{c|}{\textbf{74.06}}  & \multicolumn{1}{c|}{\textbf{57.29}}                                                      & \multicolumn{1}{c|}{59.51}           & \multicolumn{1}{c|}{40.19}                                                               & \multicolumn{1}{c|}{\textbf{70.86}}  & \multicolumn{1}{c|}{\textbf{53.12}}                                                      & \multicolumn{1}{c|}{99.55}           & \multicolumn{1}{c|}{98.80}                                                               & \multicolumn{1}{c|}{\textbf{72.80}}  & \multicolumn{1}{c|}{\textbf{56.58}}                                                      & \multicolumn{1}{c|}{69.59}           & 54.71                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{54.31}           & \multicolumn{1}{c|}{37.01}                                                               & \multicolumn{1}{c|}{75.43}           & \multicolumn{1}{c|}{64.26}                                                               & \multicolumn{1}{c|}{77.84}           & \multicolumn{1}{c|}{65.53}                                                               & \multicolumn{1}{c|}{67.35}           & \multicolumn{1}{c|}{51.53}                                                               & \multicolumn{1}{c|}{75.04}           & \multicolumn{1}{c|}{62.21}                                                               & \multicolumn{1}{c|}{91.00}           & \multicolumn{1}{c|}{85.00}                                                               & \multicolumn{1}{c|}{75.75}           & \multicolumn{1}{c|}{63.82}                                                               & \multicolumn{1}{c|}{73.82}           & 61.34                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{99.98}           & \multicolumn{1}{c|}{99.97}                                                               & \multicolumn{1}{c|}{95.74}           & \multicolumn{1}{c|}{95.64}                                                               & \multicolumn{1}{c|}{97.27}           & \multicolumn{1}{c|}{97.22}                                                               & \multicolumn{1}{c|}{98.07}           & \multicolumn{1}{c|}{98.00}                                                               & \multicolumn{1}{c|}{97.72}           & \multicolumn{1}{c|}{97.62}                                                               & \multicolumn{1}{c|}{\textbf{29.50}}  & \multicolumn{1}{c|}{\textbf{29.40}}                                                      & \multicolumn{1}{c|}{95.59}           & \multicolumn{1}{c|}{95.46}                                                               & \multicolumn{1}{c|}{87.70}           & 87.62                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.07}}   & \multicolumn{1}{c|}{\textbf{0.03}}                                                       & \multicolumn{1}{c|}{\textbf{21.91}}  & \multicolumn{1}{c|}{\textbf{18.72}}                                                      & \multicolumn{1}{c|}{77.56}           & \multicolumn{1}{c|}{72.29}                                                               & \multicolumn{1}{c|}{\textbf{31.42}}  & \multicolumn{1}{c|}{\textbf{25.51}}                                                      & \multicolumn{1}{c|}{73.30}           & \multicolumn{1}{c|}{67.25}                                                               & \multicolumn{1}{c|}{64.65}           & \multicolumn{1}{c|}{57.55}                                                               & \multicolumn{1}{c|}{73.87}           & \multicolumn{1}{c|}{67.45}                                                               & \multicolumn{1}{c|}{\textbf{48.97}}  & \textbf{44.11}                                                      \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{97.45}           & \multicolumn{1}{c|}{97.77}                                                               & \multicolumn{1}{c|}{99.64}           & \multicolumn{1}{c|}{99.77}                                                               & \multicolumn{1}{c|}{99.98}           & \multicolumn{1}{c|}{99.98}                                                               & \multicolumn{1}{c|}{99.76}           & \multicolumn{1}{c|}{99.81}                                                               & \multicolumn{1}{c|}{98.60}           & \multicolumn{1}{c|}{98.80}                                                               & \multicolumn{1}{c|}{99.49}           & \multicolumn{1}{c|}{99.58}                                                               & \multicolumn{1}{c|}{99.27}           & 99.39                                                               \\ \hline
\multicolumn{19}{|c|}{\textbf{CLIP}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{ResNet50}}}        & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{76.13}}  & \multicolumn{1}{c|}{12.89}           & \multicolumn{1}{c|}{4.21}                                                                & \multicolumn{1}{c|}{66.01}           & \multicolumn{1}{c|}{45.11}                                                               & \multicolumn{1}{c|}{71.57}           & \multicolumn{1}{c|}{48.78}                                                               & \multicolumn{1}{c|}{52.77}           & \multicolumn{1}{c|}{29.58}                                                               & \multicolumn{1}{c|}{68.58}           & \multicolumn{1}{c|}{45.41}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{72.57}           & \multicolumn{1}{c|}{50.81}                                                               & \multicolumn{1}{c|}{63.48}           & 46.27                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{7.46}            & \multicolumn{1}{c|}{2.33}                                                                & \multicolumn{1}{c|}{54.36}           & \multicolumn{1}{c|}{36.28}                                                               & \multicolumn{1}{c|}{65.68}           & \multicolumn{1}{c|}{46.18}                                                               & \multicolumn{1}{c|}{50.87}           & \multicolumn{1}{c|}{26.75}                                                               & \multicolumn{1}{c|}{59.90}           & \multicolumn{1}{c|}{38.76}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{\textbf{69.02}}  & \multicolumn{1}{c|}{\textbf{50.00}}                                                      & \multicolumn{1}{c|}{58.18}           & 42.90                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{8.18}            & \multicolumn{1}{c|}{2.94}                                                                & \multicolumn{1}{c|}{52.13}           & \multicolumn{1}{c|}{37.77}                                                               & \multicolumn{1}{c|}{65.40}           & \multicolumn{1}{c|}{48.91}                                                               & \multicolumn{1}{c|}{53.95}           & \multicolumn{1}{c|}{32.48}                                                               & \multicolumn{1}{c|}{58.28}           & \multicolumn{1}{c|}{41.19}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{99.90}                                                               & \multicolumn{1}{c|}{69.19}           & \multicolumn{1}{c|}{53.38}                                                               & \multicolumn{1}{c|}{58.16}           & 45.22                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.79}}   & \multicolumn{1}{c|}{\textbf{0.16}}                                                       & \multicolumn{1}{c|}{\textbf{15.74}}  & \multicolumn{1}{c|}{\textbf{9.10}}                                                       & \multicolumn{1}{c|}{83.52}           & \multicolumn{1}{c|}{72.38}                                                               & \multicolumn{1}{c|}{71.78}           & \multicolumn{1}{c|}{55.45}                                                               & \multicolumn{1}{c|}{82.06}           & \multicolumn{1}{c|}{69.65}                                                               & \multicolumn{1}{c|}{\textbf{84.90}}  & \multicolumn{1}{c|}{\textbf{79.20}}                                                      & \multicolumn{1}{c|}{76.16}           & \multicolumn{1}{c|}{63.29}                                                               & \multicolumn{1}{c|}{59.28}           & 49.89                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{1.14}            & \multicolumn{1}{c|}{0.86}                                                                & \multicolumn{1}{c|}{32.39}           & \multicolumn{1}{c|}{29.31}                                                               & \multicolumn{1}{c|}{\textbf{48.69}}  & \multicolumn{1}{c|}{\textbf{44.80}}                                                      & \multicolumn{1}{c|}{\textbf{26.95}}  & \multicolumn{1}{c|}{\textbf{23.71}}                                                      & \multicolumn{1}{c|}{\textbf{37.25}}  & \multicolumn{1}{c|}{\textbf{33.78}}                                                      & \multicolumn{1}{c|}{95.60}           & \multicolumn{1}{c|}{94.35}                                                               & \multicolumn{1}{c|}{69.82}           & \multicolumn{1}{c|}{66.34}                                                               & \multicolumn{1}{c|}{\textbf{44.55}}  & \textbf{41.88}                                                      \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{CLIP-ResNet50}}}   & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{59.82}} & \multicolumn{1}{c|}{10.29}           & \multicolumn{1}{c|}{4.24}                                                                & \multicolumn{1}{c|}{66.76}           & \multicolumn{1}{c|}{\textbf{46.65}}                                                      & \multicolumn{1}{c|}{75.88}           & \multicolumn{1}{c|}{\textbf{54.61}}                                                      & \multicolumn{1}{c|}{\textbf{62.65}}  & \multicolumn{1}{c|}{\textbf{39.30}}                                                      & \multicolumn{1}{c|}{70.83}           & \multicolumn{1}{c|}{\textbf{48.72}}                                                      & \multicolumn{1}{c|}{95.80}           & \multicolumn{1}{c|}{84.95}                                                               & \multicolumn{1}{c|}{80.08}           & \multicolumn{1}{c|}{\textbf{60.29}}                                                      & \multicolumn{1}{c|}{66.04}           & \textbf{48.40}                                                      \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{61.22}           & \multicolumn{1}{c|}{29.34}                                                               & \multicolumn{1}{c|}{89.52}           & \multicolumn{1}{c|}{82.55}                                                               & \multicolumn{1}{c|}{\textbf{72.28}}  & \multicolumn{1}{c|}{59.11}                                                               & \multicolumn{1}{c|}{79.53}           & \multicolumn{1}{c|}{63.79}                                                               & \multicolumn{1}{c|}{69.12}           & \multicolumn{1}{c|}{53.47}                                                               & \multicolumn{1}{c|}{75.85}           & \multicolumn{1}{c|}{67.40}                                                               & \multicolumn{1}{c|}{\textbf{77.91}}  & \multicolumn{1}{c|}{68.30}                                                               & \multicolumn{1}{c|}{75.06}           & 60.57                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{97.11}           & \multicolumn{1}{c|}{94.22}                                                               & \multicolumn{1}{c|}{94.36}           & \multicolumn{1}{c|}{92.34}                                                               & \multicolumn{1}{c|}{79.50}           & \multicolumn{1}{c|}{72.79}                                                               & \multicolumn{1}{c|}{90.14}           & \multicolumn{1}{c|}{84.56}                                                               & \multicolumn{1}{c|}{79.59}           & \multicolumn{1}{c|}{72.20}                                                               & \multicolumn{1}{c|}{\textbf{72.65}}  & \multicolumn{1}{c|}{\textbf{67.10}}                                                      & \multicolumn{1}{c|}{81.20}           & \multicolumn{1}{c|}{76.74}                                                               & \multicolumn{1}{c|}{84.94}           & 79.99                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{96.72}           & \multicolumn{1}{c|}{93.43}                                                               & \multicolumn{1}{c|}{94.68}           & \multicolumn{1}{c|}{92.71}                                                               & \multicolumn{1}{c|}{80.91}           & \multicolumn{1}{c|}{74.33}                                                               & \multicolumn{1}{c|}{91.62}           & \multicolumn{1}{c|}{86.34}                                                               & \multicolumn{1}{c|}{81.75}           & \multicolumn{1}{c|}{74.12}                                                               & \multicolumn{1}{c|}{73.25}           & \multicolumn{1}{c|}{68.10}                                                               & \multicolumn{1}{c|}{81.70}           & \multicolumn{1}{c|}{77.03}                                                               & \multicolumn{1}{c|}{85.80}           & 80.87                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.01}}   & \multicolumn{1}{c|}{\textbf{0.01}}                                                       & \multicolumn{1}{c|}{\textbf{48.30}}  & \multicolumn{1}{c|}{46.70}                                                               & \multicolumn{1}{c|}{74.95}           & \multicolumn{1}{c|}{73.15}                                                               & \multicolumn{1}{c|}{77.54}           & \multicolumn{1}{c|}{75.89}                                                               & \multicolumn{1}{c|}{\textbf{60.59}}  & \multicolumn{1}{c|}{58.38}                                                               & \multicolumn{1}{c|}{89.20}           & \multicolumn{1}{c|}{88.50}                                                               & \multicolumn{1}{c|}{84.04}           & \multicolumn{1}{c|}{83.02}                                                               & \multicolumn{1}{c|}{\textbf{62.09}}  & 60.81                                                               \\ \hline
\multicolumn{19}{|c|}{\textbf{ARCHITECTURE}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{ResNet50}}}        & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{76.13}}  & \multicolumn{1}{c|}{12.89}           & \multicolumn{1}{c|}{4.21}                                                                & \multicolumn{1}{c|}{66.01}           & \multicolumn{1}{c|}{45.11}                                                               & \multicolumn{1}{c|}{71.57}           & \multicolumn{1}{c|}{48.78}                                                               & \multicolumn{1}{c|}{52.77}           & \multicolumn{1}{c|}{29.58}                                                               & \multicolumn{1}{c|}{68.58}           & \multicolumn{1}{c|}{45.41}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{72.57}           & \multicolumn{1}{c|}{50.81}                                                               & \multicolumn{1}{c|}{63.48}           & 46.27                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{7.46}            & \multicolumn{1}{c|}{2.33}                                                                & \multicolumn{1}{c|}{54.36}           & \multicolumn{1}{c|}{36.28}                                                               & \multicolumn{1}{c|}{65.68}           & \multicolumn{1}{c|}{46.18}                                                               & \multicolumn{1}{c|}{50.87}           & \multicolumn{1}{c|}{26.75}                                                               & \multicolumn{1}{c|}{59.90}           & \multicolumn{1}{c|}{38.76}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{100.00}                                                              & \multicolumn{1}{c|}{\textbf{69.02}}  & \multicolumn{1}{c|}{\textbf{50.00}}                                                      & \multicolumn{1}{c|}{58.18}           & 42.90                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{8.18}            & \multicolumn{1}{c|}{2.94}                                                                & \multicolumn{1}{c|}{52.13}           & \multicolumn{1}{c|}{37.77}                                                               & \multicolumn{1}{c|}{65.40}           & \multicolumn{1}{c|}{48.91}                                                               & \multicolumn{1}{c|}{53.95}           & \multicolumn{1}{c|}{32.48}                                                               & \multicolumn{1}{c|}{58.28}           & \multicolumn{1}{c|}{41.19}                                                               & \multicolumn{1}{c|}{100.00}          & \multicolumn{1}{c|}{99.90}                                                               & \multicolumn{1}{c|}{69.19}           & \multicolumn{1}{c|}{53.38}                                                               & \multicolumn{1}{c|}{58.16}           & 45.22                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{0.79}}   & \multicolumn{1}{c|}{\textbf{0.16}}                                                       & \multicolumn{1}{c|}{\textbf{15.74}}  & \multicolumn{1}{c|}{\textbf{9.10}}                                                       & \multicolumn{1}{c|}{83.52}           & \multicolumn{1}{c|}{72.38}                                                               & \multicolumn{1}{c|}{71.78}           & \multicolumn{1}{c|}{55.45}                                                               & \multicolumn{1}{c|}{82.06}           & \multicolumn{1}{c|}{69.65}                                                               & \multicolumn{1}{c|}{\textbf{84.90}}  & \multicolumn{1}{c|}{\textbf{79.20}}                                                      & \multicolumn{1}{c|}{76.16}           & \multicolumn{1}{c|}{63.29}                                                               & \multicolumn{1}{c|}{59.28}           & 49.89                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{1.14}            & \multicolumn{1}{c|}{0.86}                                                                & \multicolumn{1}{c|}{32.39}           & \multicolumn{1}{c|}{29.31}                                                               & \multicolumn{1}{c|}{\textbf{48.69}}  & \multicolumn{1}{c|}{\textbf{44.80}}                                                      & \multicolumn{1}{c|}{\textbf{26.95}}  & \multicolumn{1}{c|}{\textbf{23.71}}                                                      & \multicolumn{1}{c|}{\textbf{37.25}}  & \multicolumn{1}{c|}{\textbf{33.78}}                                                      & \multicolumn{1}{c|}{95.60}           & \multicolumn{1}{c|}{94.35}                                                               & \multicolumn{1}{c|}{69.82}           & \multicolumn{1}{c|}{66.34}                                                               & \multicolumn{1}{c|}{\textbf{44.55}}  & \textbf{41.88}                                                      \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{ViT-B-16}}}        & \multicolumn{1}{c|}{\textbf{MSP}}                      & \multicolumn{1}{c|}{\multirow{5}{*}{81.07}} & \multicolumn{1}{c|}{21.54}           & \multicolumn{1}{c|}{10.09}                                                               & \multicolumn{1}{c|}{58.30}           & \multicolumn{1}{c|}{41.28}                                                               & \multicolumn{1}{c|}{68.68}           & \multicolumn{1}{c|}{\textbf{49.68}}                                                      & \multicolumn{1}{c|}{51.52}           & \multicolumn{1}{c|}{32.03}                                                               & \multicolumn{1}{c|}{66.56}           & \multicolumn{1}{c|}{\textbf{48.08}}                                                      & \multicolumn{1}{c|}{95.65}           & \multicolumn{1}{c|}{91.30}                                                               & \multicolumn{1}{c|}{71.31}           & \multicolumn{1}{c|}{\textbf{53.54}}                                                      & \multicolumn{1}{c|}{61.94}           & 46.57                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{MaxLogit}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{18.52}           & \multicolumn{1}{c|}{8.23}                                                                & \multicolumn{1}{c|}{54.84}           & \multicolumn{1}{c|}{38.09}                                                               & \multicolumn{1}{c|}{69.14}           & \multicolumn{1}{c|}{52.49}                                                               & \multicolumn{1}{c|}{52.26}           & \multicolumn{1}{c|}{33.03}                                                               & \multicolumn{1}{c|}{66.89}           & \multicolumn{1}{c|}{49.91}                                                               & \multicolumn{1}{c|}{82.90}           & \multicolumn{1}{c|}{72.60}                                                               & \multicolumn{1}{c|}{\textbf{70.17}}  & \multicolumn{1}{c|}{54.13}                                                               & \multicolumn{1}{c|}{59.25}           & 44.07                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{Energy}}                   & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{24.15}           & \multicolumn{1}{c|}{13.50}                                                               & \multicolumn{1}{c|}{57.39}           & \multicolumn{1}{c|}{46.01}                                                               & \multicolumn{1}{c|}{74.31}           & \multicolumn{1}{c|}{65.24}                                                               & \multicolumn{1}{c|}{64.08}           & \multicolumn{1}{c|}{50.90}                                                               & \multicolumn{1}{c|}{72.77}           & \multicolumn{1}{c|}{62.80}                                                               & \multicolumn{1}{c|}{\textbf{68.65}}  & \multicolumn{1}{c|}{62.20}                                                               & \multicolumn{1}{c|}{73.77}           & \multicolumn{1}{c|}{63.99}                                                               & \multicolumn{1}{c|}{62.16}           & 52.09                                                               \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{ViM}}                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{2.34}}   & \multicolumn{1}{c|}{\textbf{0.85}}                                                       & \multicolumn{1}{c|}{\textbf{43.94}}  & \multicolumn{1}{c|}{\textbf{31.49}}                                                      & \multicolumn{1}{c|}{\textbf{61.12}}  & \multicolumn{1}{c|}{50.35}                                                               & \multicolumn{1}{c|}{\textbf{17.77}}  & \multicolumn{1}{c|}{\textbf{10.66}}                                                      & \multicolumn{1}{c|}{\textbf{59.46}}  & \multicolumn{1}{c|}{49.05}                                                               & \multicolumn{1}{c|}{72.90}           & \multicolumn{1}{c|}{\textbf{61.80}}                                                      & \multicolumn{1}{c|}{71.58}           & \multicolumn{1}{c|}{58.70}                                                               & \multicolumn{1}{c|}{\textbf{47.01}}  & \textbf{37.56}                                                      \\ \cline{2-2} \cline{4-19} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{c|}{\textbf{GradNorm}}                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{96.13}           & \multicolumn{1}{c|}{96.43}                                                               & \multicolumn{1}{c|}{92.87}           & \multicolumn{1}{c|}{93.14}                                                               & \multicolumn{1}{c|}{96.70}           & \multicolumn{1}{c|}{96.91}                                                               & \multicolumn{1}{c|}{95.56}           & \multicolumn{1}{c|}{95.93}                                                               & \multicolumn{1}{c|}{96.85}           & \multicolumn{1}{c|}{97.05}                                                               & \multicolumn{1}{c|}{98.65}           & \multicolumn{1}{c|}{98.75}                                                               & \multicolumn{1}{c|}{97.86}           & \multicolumn{1}{c|}{98.04}                                                               & \multicolumn{1}{c|}{96.38}           & 96.61                                                               \\ \hline
\end{tabular}}
\label{table5}
\end{sidewaystable}
